ABO: Abandon Bayer Filter for Adaptive Edge Offloading in Responsive Augmented Reality

Bayer-patterned color filter array (CFA) has been the go-to solution for color image sensors. In augmented reality (AR), although color interpolation (i.e., demosaicing) of pre-demosaic RAW images facilitates a user-friendly rendering, it creates no benefits in offloaded DNN analytics but increases the image channels by 3 times inducing higher transmission overheads. The potential optimization in frame preprocessing of DNN offloading is yet to be investigated. To that end, we propose ABO, an adaptive RAW frame offloading framework that parallelizes demosaicing with DNN computation. Its contributions are three-fold: First, we design a configurable tile-wise RAW image neural codec to compress frame sizes while sustaining downstream DNN accuracy under bandwidth constraints. Second, based on content-aware tiles-in-frame selection and runtime bandwidth estimation, a dynamic transmission controller adaptively calibrates codec configurations to maximize the DNN accuracy. Third, we further optimize the system pipelining to achieve lower end-to-end frame processing latency and higher throughput. Through extensive evaluations on a prototype platform, ABO consistently achieves 40% more frame processing throughput and 30% less end-to-end latency while improving the DNN accuracy by up to 15% than SOTA baselines. It also exhibits improved robustness against dim lighting and motion blur situations.

==> comment/1_intro.tex <==
\section{Introduction} \label{sec1}

% background
Augmented reality (AR) overlays digital content like images, videos, and sounds onto the real-world environment, enhancing human-environment interactions by adding generated elements.
It has extensive applications in surgical assistance~\cite{shenai2011virtual,chinzei2000mr}, E-commerce~\cite{lu2007augmented,yim2017augmented}, gaming~\cite{ananthanarayanan2017real,piekarski2002arquake}, and education~\cite{yuen2011augmented,wu2013current}. 
Accurate perception of physical objects in real-time lays the foundational pillars for AR.
While deep neural networks (DNN) have greatly enhanced machine perception capabilities (\eg object detection), their computation-intensive nature incurs significant challenges to limited compute resources on mobile AR devices. 
Thus, edge offloading that transmits data to a nearby edge server for remote DNN analytics has become a leading solution~\cite{eshratifar2018energy,kang2017neurosurgeon}.

% AR requirements and objectives 
% \zmz{finetune logic}
The human-device-environment interactions in AR call for low response latency (< 40 ms), high processing throughput (> 25 FPS\cite{24fps}), and sufficient task accuracy for a \textit{responsive}, \textit{smooth}, and \textit{precise} service. 
% In edge offloading, both the onboard processing workload and wireless data transmission should be optimized to fulfill the above service-level objectives (SLO).
% To save frame transmission time, the captured frames are first compressed by an \textit{image codec} before transmission, which should effectively reduce image sizes, run efficiently on mobile devices, and dynamically adapt to bandwidth fluctuations.
% Standard image codecs like JPEG, originally optimized for human browsing, could be suboptimal in serving DNN model analytics. 
% \zmz{\textbf{not necessary here with two sentences.} Specifically, we consider object detection as the offloaded visual task which lays the foundation of many AR applications~\cite{arvr1,arvr2}.
% The objectives drive us to rethink the design of offloading frameworks appropriate for AR applications.}
% Bayer filter process
The end-to-end response latency denotes the duration from a frame being captured to DNN inference results being rendered, including frame preprocessing, data compressing (\ie encoding), two-way transmission, remote DNN inference, and rendering. 
To save network bandwidth, the captured frames are first compressed by an \textit{image codec} before transmission. It should substantially reduce frame sizes, run efficiently on mobile devices, and dynamically adapt to bandwidth fluctuations.
% We observe that JPEG and most works~\cite{minnen2020channel,mentzer2020high,cheng2020learned} focus on encoding RGB images, but overlook potential optimizations in image preprocessing.
Standard image codecs like JPEG, and recent offloading approaches~\cite{minnen2020channel,mentzer2020high,cheng2020learned}, all focus on encoding demosaiced RGB frames and overlook potential optimizations in preprocessing.
Besides, they are optimized for human browsing experience and could be suboptimal in serving DNN analytics.

% pre-demosaicing motivation
Common image sensors use Bayer-patterned color filter array (CFA) to capture color information into single-channel \textit{RAW frames}, which are then \textit{demosaiced} to interpret real-world colors into 3-channel \textit{RGB frames}. 
Demosaicing high-resolution frames can take more than 25 ms on resource-constrained edge devices (\eg NVIDIA Jetson Nano), occupying a large portion of end-to-end latency since the remaining steps only take below 30 ms in total.
We believe demosaicing is only essential to rendering frames into a viewable form but can be skipped for DNN inference.
Since RGB images are solely interpolated from RAW ones without any extra input, RAW images should provide a similar task accuracy when feeding into the downstream DNN model despite having less data.
We are thereby interested in utilizing RAW frames in edge offloading for DNN analytics.
It enables decoupling offloading and demosaicing with no resource contentions (\ie communication vs. computation), thus the onboard demosaicing overhead can be hidden in parallel pipelines, leading to lower latency and higher throughput.

% % pre-demosaicing motivation
% We claim that demosaicing is only part of the essential pipeline to render images into a viewable format, but is not necessary for DNN analytics.
% Since RGB images are interpolated from RAW images without extra information input, RAW images should provide a similar task accuracy when used as input of the downstream DNN model despite their smaller sizes.
% We thereby are interested in enabling RAW image-based DNN offloading to optimize the end-to-end responsiveness of edge offloading.
% It helps decouple the offloading and demosaicing processes that do not have resource contentions, thus the onboard demosaicing overhead can be hidden from the parallel offloading pipeline.

% challenges
% The following technical challenges make the decouple non-trivial:
However, there are three technical challenges in the decoupled pipelines:
% First, an effective codec is needed that can compress RAW images no larger than JPEG files but achieve a higher downstream DNN accuracy after decoding.
First, an efficient codec is required to compress RAW frames no larger than JPEG files, while ensuring higher downstream DNN accuracy upon decoding.
Second, to prioritize real-time interactions, we need to dynamically calibrate the configuration of the codec with accuracy-efficiency tradeoffs in response to runtime bandwidth fluctuations.
Third, we need to make both the encoder and the adaptation controller lightweight enough to execute efficiently on edge devices without incurring excessive overhead.

To that end, we propose \model, an adaptive pre-demosaic RAW frame edge offloading framework for DNN analytics, that decouples demosaicing from the offloading into parallel processes, providing real-time responses under constrained and dynamic network bandwidth. 
Its design includes three key perspectives.
% 
% \zmz{\textbf{compress these paragraphs into one paragraph.} First, we train a configurable neural codec that operates in the granularity of sub-frame image tiles. 
% It constitutes an asymmetric autoencoder, with a single-layer encoder deployed on the edge device to quickly compress the RAW tiles, and a multi-layer decoder is deployed on the edge server for reconstruction.
% Similar to DeepCOD~\cite{yao2020deep}, it uses server-side computation in exchange for bandwidth savings.
% The autoencoder is trained to minimize both the image reconstruction error for semantic intactness and the downstream DNN loss through knowledge distillation to enhance task awareness.
% Besides, the neural codec is designed to be highly configurable where the tiles-in-frame to encode and the dimensions of compressed features can both be calibrated.
% 
% Second, we design a dynamic transmission controller that adaptively decides which tiles of which frames to encode according to video content, and further decide the configuration of encoding based on selected tiles and estimated bandwidth through a lightweight estimator, to maximize the downstream DNN task accuracy without violating the real-time constraint.  
% 
% Third, we implement and optimize the system pipeline for the offloading framework, by allocating rendering and offloading into parallel threads to optimize the resource utilization. The system is implemented on a 3D-printed prototype platform with Jetson Nano as the client device and a desktop with RTX 4090 as the edge server.}
First, we train a configurable RAW image neural codec that operates on sub-frame image tiles with an asymmetric autoencoder (\ie device-side shallow encoder and server-side deep decoder) to quickly compress RAW tiles and utilize server-side computation in exchange for transmission savings.
It is trained in a task-aware manner by minimizing both the image reconstruction loss and knowledge distillation loss from downstream DNN, and it is highly configurable in tiles-in-frame selections and the encoded feature dimensions. 
% 
Second, we design a dynamic transmission controller that adaptively decides the two configuration knobs based on real-time video content and estimated bandwidth, to maximize the downstream task accuracy without violating the real-time latency constraint. 
% 
Third, we refactor the system pipeline by decoupling and parallelizing demosaicing and offloading processes to optimize bottleneck resource utilizations (\ie device-side GPU and wireless network).

\begin{figure}[t!]
    \centering
    \includegraphics[width=0.8\linewidth]{figure/2/2-2-v4.pdf}
    \vspace{-0.3cm}
    \caption{Comparing two image transmission types.}
    \label{fig:offload}
\end{figure}

% evaluation 
We extensively evaluate the performance of \model with datasets collected with a prototype AR system. The results show that \model outperforms not only JPEG but also SOTA baselines, with up to 15\% improvement on downstream DNN accuracy while incurring similar bandwidth consumption. Meanwhile, the dynamic offloading pipeline of \model consistently provides over 40\% more throughput and 30\% less response latency, being the only one that achieved the target of real-time experience.
% \shengzhong{Include the response latency savings.}

Our main contributions are summarized as follows:
\begin{itemize}
    \item We are the first to decouple the visual DNN offloading from image demosaicing such that they can run in parallel for higher throughput and lower end-to-end latency.
    \item We design a tile-based configurable neural codec for RAW images to achieve different latency-accuracy tradeoffs.
    \item We propose an adaptation controller algorithm to optimize the offloaded DNN task accuracy and frame processing throughput upon network bandwidth fluctuations.
    \item We implement both the hardware and software prototype system and perform extensive evaluations to demonstrate the effectiveness and efficiency of \model.
\end{itemize}





==> comment/2_background.tex <==
\section{Background and Motivations}
\label{sec2}

% This section reviews preliminary background knowledge on DNN offloading and digital image processing, as well as the main motivations driving this paper.

\subsection{DNN Offloading for Augmented Reality}
% DNN analytics in AR --> offloading
DNN analytics (\eg object detection) are crucial in AR applications as they enhance the interactions between digital content and users by helping anchor virtual elements to real-world objects. 
Due to limited onboard resources, offloading computation-intensive DNN tasks to a nearby edge server has been a common practice~\cite{offloadsurvey}: The DNN model loaded on the server processes frames uploaded from the client device. The detection results are then sent back to the client for user-facing rendering.
An offloading pipeline needs to support high-resolution frame processing with high throughput in real time for a responsive, smooth, and accurate user experience.

\begin{figure}[t!]
    \centering
    \includegraphics[width=1.0\linewidth]{figure/2/2-1-mod.pdf}
    \caption{Typical on-sensor image processing pipeline.}
    \label{fig:demosaic}
\end{figure}

To save bandwidth consumption, standard image codecs (\eg JPEG) are applied on the client to compress frames before transmission, which actually mismatch with DNN inference needs.
As shown in Figure~\ref{fig:offload}, we distinguish two transmission types:
\begin{itemize}
    \item In \textbf{human-centric transmission} like content delivery networks, frames are transmitted for human viewing after decoding with standard codecs optimized for human viewing.
    \item In \textbf{machine-centric transmission}, the decoded frames are processed by DNN models, thus downstream model accuracy should guide the codec designing.
\end{itemize}
As a solution, the image codec should be refactored to align with the downstream DNN inference and abandon any information unrelated to DNN prediction (\ie interpolated colors, content intactness). 
Besides, the human-in-the-loop nature of AR calls for both \textit{low latency} and \textit{high throughput}. 
% Specifically, low latency requires durations between image capturing, to DNN offloading, until rendering to be as short as possible, which is critical to reduce the lag between user actions and virtual reactions.
% High throughput requires more frames to be processed per second to guarantee smooth viewing experiences.
Low latency provides responsiveness, while high throughput guarantees smoothness.

\subsection{Demosaicing in Digital Image Processing}
\label{sec2-1}

Bayer filter is a CFA placed over the photodiode array for capturing images with color. As shown in Figure~\ref{fig:demosaic}, a typical CFA pattern is a 2x2 repeating unit (RGGB filter cell), and it outputs single-channel \textit{RAW images}. 
% The green filters are more prevalent because the luminance perception of the human retina uses M and L cone cells combined during daylight vision, which are most sensitive to green light~\cite{retina-0,retina-1}. 
% Each pixel on the camera sensor only captures one RGB color, depending on the filter it is covered by. 
% The outcome is a single-channel \textit{raw Bayer image} (\textit{RAW image} for short). 
% To reconstruct the colorful image, the demosaicing algorithms are applied~\cite{demosaic-0,demosaic-1,demosaic-2} to estimate the missing pixel colors based on nearby pixels and generate \textit{RGB images} with the same spatial dimensions in 3 color channels.
% This process is called the \textit{demosaicing}, which takes around 25 to 45 ms on embedded platforms (\ie Nvidia Jetson Nano), depending on the pixel count.
To reconstruct them into the RGB form, demosaicing algorithms are applied~\cite{demosaic-0,demosaic-1,demosaic-2} to estimate the missing color channels based on nearby pixels, which takes 25 to 45 ms on embedded platforms (\ie Nvidia Jetson Nano, software-based solution, details in Appendix\ref{apdx:softvshard}).
% In a typical AR offloading pipeline, the reconstructed RGB images are compressed through standard image codecs (\eg JPEG) to reduce the bandwidth consumption in wireless transmission. 
% However, according to information theory~\cite{gallager1968information},
% no extra information is generated without extra input. 
Although demosaiced 3-channel RGB images facilitate human browsing, they do not lead to better DNN inference performance but result in higher transmission overhead. 
% Instead, demosaiced 3-channel RGB images result in higher transmission overhead than single-channel RAW images.
Thus the RAW images, with appropriate codecs, could be better candidates for DNN offloading.
% Besides, when the dependency between offloading and demosaicing is removed, they can run in parallel consuming different resource types (network vs. computation) before rendering the RGB images with returned DNN prediction results.

\input{table/tab1_accuracy_bandwidth_tradeoff}

\begin{figure}[t!]
    \centering
    \vspace{0.3cm}
    \includegraphics[width=\linewidth]{figure/2/2-1-2.pdf}
    \vspace{-0.5cm}
    \caption{Comparison of the original RAW image, \model-noDistill decoded image and \model-Distill decoded image with edge clearness values (Definitions given in Appendix~\ref{apdx:clearness}). All images are demosaiced to RGB formats for better viewing.}
    \label{fig:diff-comparison}
\end{figure}

 

We conduct experiments to validate the hypothesis. 
Using object detection as the offloaded task, we first train two YOLO models~\cite{yolo} on RAW and RGB images of the same dataset (details in Appendix~\ref{apdx:rawdataset}).
% \footnote{Common image datasets do not contain RAW format before demosaicing. We need to use dedicated camera sensors to collect data to preserve RAW images and demosaiced RGB images. More details about the dataset are introduced in Section~\ref{rawdataset}}. 
% The model architecture and training hyper-parameters are all fixed. 
We then evaluate the RGB model on RGB and JPEG-decoded images while evaluating the RAW model on RAW and \model-decoded images, respectively. 
% To see if using a RAW image with a grid-like RGB pattern instead of a common layered RGB form will interfere with the function of downstream vision tasks, we verify such suspicion by training the YOLO model using the best quality. For RAW images, there is neither codec nor compression for RAW, For JPEG, the quality configuration parameter is set to 100 for JPEG. 
% 
The results in Table~\ref{tab:t1} show that (1) Demosaicing does not enhance the downstream task performance. Instead, the samplings of real-world information remain original and intact in RAW images, which receive better object detection performance than interpolated RGB images (RAW vs. RGB). 
(2) Without encoding, both frame types lead to excessive frame sizes intolerable for transmission, while \model and JPEG can effectively reduce the transmitted frame sizes.
% As a mature image codec, JPEG leads to negligible accuracy degradation compared to RGB.
(3) Although \model causes a small degradation in model accuracy (\model-noDistill vs. RAW), finetuning its codec through knowledge distillation 
% from the downstream YOLO model 
achieves even slightly better performance than RAW (\model-Distill vs. RAW).

We visualize the different image types in Figure~\ref{fig:diff-comparison}, and find knowledge distillation achieves targeted image-enhancing artifacts in a mission-oriented manner with better exposed object outlines.
% and distinguishable background patterns. 
\model achieves lower bandwidth consumption than JPEG without accuracy degradation, thus presenting higher offloading potential.
% However, unlike JPEG, RAW images do not have an effective compression method, meaning that the size of a frame is determined purely by the amount of pixels and the bit depth of sampling. In high-resolution scenario like AR/VR system, such character will cause unexpected overhead. For instance, our camera has 3072*2048 pixels and an 8-bit depth of sampling, resulting in a huge 6MB frame size for just one frame, which is not usable for storage or transmission. How to immensely shrink the size of a frame without harming task performance will be one of the major challenges in \model.

\subsection{Pre-Demosaic Offloading Savings}
Existing offloading frameworks~\cite{yao2020deep,li2020reducto,liu2019edge,xie2019source} only optimize the latency from demosaiced RGB images to results rendering but overlook the latency associated with onboard demosaicing. %\shengzhong{Add references.}
One main motivation of this paper is to decouple \textit{image offloading} and \textit{demosaicing} for efficiency savings. 
% Having analyzed its feasibility from the accuracy perspective, here we analyze its efficiency savings.
% 
% Specifically, we compare the standard serialized offloading procedure using JPEG and the proposed ABO procedure performing image encoding and transmission using RAW images such that onboard demosaicing can run in parallel to the transmission and remote DNN analytics. 
We compare the standard JPEG-based offloading process with the RAW-based ABO process, which allows onboard demosaicing to run in parallel with transmission and remote DNN analysis.
We use an Nvidia Jetson Nano as the edge device and a desktop with Nvidia RTX 4090 GPU as the edge server, whose results are reported in Figure~\ref{fig:timeline}. 
With the decoupled threads, the execution overhead on demosaicing (\ie 25 ms) is hidden behind image offloading steps.
Besides, as indicated in Table~\ref{tab:t1}, single-channel RAW images result in smaller sizes, reducing the network transmission latency.
The end-to-end frame processing latency is reduced from 54 ms to 37 ms, fulfilling the real-time requirement of 40 ms. Its frame throughput increases to over 27 FPS, surpassing the 25 FPS threshold for human viewing.
% To conclude, performing pre-Bayer offloading enables effective multi-thread pipelining and bandwidth saving, thus significantly improving both latency and throughput metrics.
% All inspiring findings motivate us to design \model.
% However, the immense number of pixels that need to be computed in a high-resolution scenario will be a struggle for low-power-consumption client devices. And if the pipeline is latency sensitive and needs to be operated in real-time (typically meaning over 25FPS), like AR/VR system, the time overhead caused by debayer and resize process might be unacceptable. As illustrated in Figure~\ref{fig:timeline}, the processing time for one frame needs to be under 40ms if a system can be described as real-time. But the debayer and resizing process is taking over 23ms to run which is over 50\% of the required frame time and finally making the system fail to meet the requirement. 

% If using RAW instead of debayered RGB frames, the system can be designed in a multi-threaded manner instead of being strictly sequential. That is, the time overhead of other processes like encoding and transmission can be hidden in the time of color interpretation. The challenge here is how to make the encoding of RAW images run fast enough to meet the real-time throughput requirement while balancing downstream vision task performance and bandwidth consumption.

\begin{figure}[t!]
    \centering
    \includegraphics[width=0.9\linewidth]{figure/2/timeline.pdf}
    \vspace{-0.3cm}
    \caption{Frame processing time comparison between \textit{serialized procedure in JPEG} and \textit{pipelined procedure in \model}.}
    \label{fig:timeline}
    \vspace{0.2cm}
\end{figure}

==> comment/3_framework.tex <==
\section{\model~Framework} 
\label{sec:framework}
% We first give an overview of the proposed \model framework, then introduce its major components with design details.

% \shengzhong{The general purpose of this section: 1) Align with the insights in the introduction; 2) Address the missing details of each component that are not included in the introduction.}

\begin{figure}[t!]
    \centering
    \includegraphics[width=1\linewidth]{figure/3/3-1-mod5.pdf}
    \vspace{-0.6cm}
    \caption{\model framework overview.}
    \label{fig:overview}
\end{figure}

\begin{figure*}[t!]
    \centering
    \includegraphics[width=0.85\linewidth]{figure/3/tiles.pdf}
    \caption{The tile-wise encoding of \model with tile-in-frame selection and multiple encoding configurations.}
    \label{fig:tiles}
\end{figure*}

\subsection{Overview}
% \shengzhong{In the overview, we need to explain 1) how many components we have; 2) what is the task of each component; 3) what is the operation workflow of the whole framework. Essentially, at the high level, you need to well explain your Figure 5 in this subsection (including the main modules and the arrows between the modules), while also keeping the overview short.}
The overview of \model is summarized in Figure~\ref{fig:overview}, which includes two main components: a \textit{tile-wise RAW image neural codec} with different configurations to be calibrated with, and a \textit{dynamic transmission controller} tackling bandwidth fluctuations.

\textbf{Tile-wise RAW Image Neural Codec:}
It consists of a lightweight encoder on the edge device to compress sub-frame RAW image tiles into feature maps with compressed sizes, and a deep decoder on the edge server to reconstruct the RAW image from transmitted feature maps for DNN inference. Multiple encoding configurations are available to balance the offloaded DNN accuracy and bandwidth consumption during the transmission.

\textbf{Dynamic Transmission Controller:}
Given a RAW frame, it first selects the tiles that may contain objects, then determines the codec configuration based on the estimated bandwidth and selected image tiles, adapting to dynamically fluctuating networks.


\subsection{Tile-wise RAW Image Neural Codec}
\label{sec3-2}
% \shengzhong{Need a diagram to visualize the tile/block-based compression idea. Do not address the ``adaptive'' here, but instead address that your codec supports dynamic configuration under different bandwidth constraints.}
A neural codec is expected to significantly reduce the frame size through encoding while effectively sustaining the downstream DNN accuracy on decoded output.
\model's neural codec design is based on two ideas:
First, \model reduces the client-side computation by deploying single-layer neural encoders on edge devices and heavyweight neural decoders on edge servers.
% Considering the resource-rich nature of edge servers, the decoder computation can also finish in a short time.
Second, instead of encoding a high-resolution RAW image as a whole, \model separately encodes individual sub-frame tiles and provides multiple encoder configurations, both constituting a tunable space for codec calibration upon bandwidth dynamics.

% \shengzhong{addresses: 1) we have asymmetric encoder-decoder design; 2) how we support dynamic configuration (on the encoder and the first layer of the decoder)}

% \shengzhong{Use a paragraph to explain how the design points correspond to each of our objectives of neural codec mentioned in the introduction before we introduce each design point.}

% \shengzhong{Within your explanation, do not use concrete numbers (\eg 3 blocks in a row and 4 blocks in a column). Instead, you should say the whole frame is partitioned as a grid of $M\times K$ tiles with xx\% overlaps at each dimension. Do not say your channels are set as 8 or 4, but instead say you have multiple choices of encoded output channels. Leave the instantiation of these concrete parameters into the first subsection of your experiment (\ie experimental setup). Since we do not have enough space, consider moving these instantiations to the Appendix.}

\subsubsection{Asymmetric Configurable Autoencoder.}
% \shengzhong{Introduce the encoder-decoder architecture and address the fact the encoder is very lightweight to run on edge devices, and we have separate encoders for different encoders for optimized accuracy, without much higher memory overhead. Address most parameters are shared for different configurations except two layers, such that we achieve optimized accuracy at the cost of low memory overhead.}
The neural codec of \model is designed to be asymmetric. 
The encoder only includes a single convolution layer for compressing tile spatial dimensions.
The kernel stride and numbers of output channels are different for each configuration (with parameters separately assigned).
The single convolution layer design can run in real-time on edge devices, while multiple encoders only induce reasonable memory overhead.
On the other hand, The decoder on the edge server (assumed to be resource-rich) has a much larger scale to secure the reconstruction quality.
The basic decoder structure is a stack of residual blocks\cite{he2016deep} (details in Appandix~\ref{apdx:modeulstructure}).
To cope with heterogeneous encoding configurations without hosting multiple deep decoders, as shown in Figure~\ref{fig:tiles}, we use a pluggable design: Each encoder configuration has a separate decoder head to unify the feature map dimensions. After that, all configurations share the same decoder layers until the output.
All encoder-decoder configurations are trained jointly to enhance their compatibility within the shared decoder parameters.
% \red{add details of decoder}
% To maximize task accuracy under different bandwidth restraints, multiple choices of codec configuration have been provided. Different configurations are controlled by the width and depth of the encoder (the stride steps of convolution and the number of output channels, specifically), inspired by EfficientNet\cite{tan2019efficientnet}. 
% Configurations with larger parameters provide higher task accuracy, while smaller configurations provide lower bandwidth consumption with minor task accuracy degradation. 
% The configurations are designed to be resource-saving and low-overhead since they need to be loaded onto the client device simultaneously.
% To reduce resource wasting, most parameters of the codec are shared except the encoders and the first layer of the decoder among all the configurations.

\subsubsection{Frame Color Preservation}
If a RAW frame is fed into the encoder in the original 1-channel format, the grid-patterned RGB information would be erased by the convolution kernel, hard to recover the color information. Instead, we disassemble a RAW frame by the color channels in the CFA repeating pattern and stack the four disassembled channels to create a 4-channel input (illustrated in Figure~\ref{fig:4into1}), so that the mosaiced color information can be preserved during the encoding-decoding processes. 
However, though a disassembled 4-channel and the original 1-channel frames have the same pixel volume and information, the spatial information of a 4-channel input is downsampled by $2\times$ at each dimension which will greatly degrade the extracted high-level spatial features of the DNN model\cite{tan2019efficientnet}.
Thus, the decoded tiles need to be reassembled into the original 1-channel format according to the CFA pattern before feeding into the downstream model.

\subsubsection{Tile Partitioning.}
Object detection models are highly spatially localized in feature extraction, meaning the detection quality will not be affected by removing unrelated background areas. 
Furthermore, selectively transmitting task-related subframe areas helps greatly reduce bandwidth consumption. 
To achieve this, we evenly split a frame as a grid of $r\times c$ tiles with overlap to preserve the reconstruction quality from tile padding artifacts. 
After transmitting the selected tiles with positional indexes to the edge server, the decoded tiles will be placed at their original position in an empty frame canvas filled with default pixel colors. 
% Given that selected tiles $\bm{\{T_1,T_2,\cdots,T_n\}}$ are at the $\bm{\{r_1,r_2,\cdots,r_n\}}$ row and the $\bm{\{c_1,c_2,\cdots,c_n\}}$ column of the original frame respectively, and denote the encoded tiles to be $\bm{\{T^e_1,T^e_2,\cdots,T^e_n\}}$, then the transmitted data will be $\bm{\{T^e_1,T^e_2,\cdots,T^e_i,[(c_1,r_1),(c_2,r_2),\cdots,(c_n,r_n)]\}}$. Denote the decoded tiles as $\bm{\{T^d_1,T^d_2,\cdots,T^d_n\}}$, then $\bm{T^d_i}$ will be inserted into the $\bm{c_i}$ column of the $\bm{r_i}$ row of the prepared empty frame which will be the input of downstream DNN visual model.
% The selected tiles are grouped into a batch for parallel encoding and decoding, while the decoded tiles are assembled into a canvas with missing tiles filled with default pixel colors.

\subsubsection{Learning Objectives.}
% \shengzhong{Address that we use both MSE loss and knowledge distillation loss in learning the autoencoders of codec. Use equations to explain each objective. Explain how to we weigh over different configurations.}
The neural codec training is divided into two phases.
The first phase only focuses on the reconstruction quality by minimizing a mean-squared error (MSE) loss between the original input and the decoded output. 
% However, the purpose of a machine-centric system is not a higher perceptual image quality but a better task performance. 
In the second phase, we introduce knowledge distillation~\cite{distill} from the downstream DNN model to enhance the preservation of task-related information, achieving higher accuracy in the downstream task.
The frozen downstream model is concatenated to the decoded output and its task loss (\ie object detection loss) is backpropagated to both the encoder and decoder during their update.
Besides, in the distillation phase, losses from different coding configurations are weighted by the proportion of their original MSE losses.
% Assume there are $\bm{m}$ train samples in total, and $\bm{y_i}$ is the codec output of corresponding train sample $\bm{x_i}$. Then the MSE loss can be described as
% \begin{equation}
% Loss_{MSE}=\frac{1}{n}\sum_{i=1}^{n}(x_i-y_i)^2.
% \end{equation}
Assume there are $\bm{n}$ codec configurations in total, and denote the MSE loss of one of the configurations as $\bm{\{Loss_{MSE}\}_i}$, the weight for this configuration can be described as:
\begin{equation}
w_i=\frac{\sum_{i=1}^{n}\{Loss_{MSE}\}_i}{\{Loss_{MSE}\}_i}.
\end{equation}
Denote the loss function of downstream DNN visual model as $\bm{Loss_{task}}$, so that the task loss of configuration $i$ is $\bm{\{Loss_{task}\}_i}$, and the knowledge distillation loss is:
\begin{equation}
Loss_{KD}=\sum_{i=1}^{n}w_i*\{Loss_{task}\}_i,
\end{equation}
where $\bm{Loss_{task}}$ depends on the used downstream model. 
In this way, all codec configurations have the same loss value at the beginning of knowledge distillation, with the intuition of forcing them to be updated at a similar rate.

\begin{figure}
    \centering
    \includegraphics[width=0.9\linewidth]{figure/3/4into1_v2.pdf}
    \vspace{-0.3cm}
    \caption{Color-preserving input preprocessing.}
    \label{fig:4into1}
\end{figure}

\subsection{Dynamic Transmission Controller}
\label{sec3-3}
% One of the biggest challenges in typical AR scenarios is the fluctuating and limited bandwidth due to the uncertainty of wireless connection. 
To cope with network fluctuations, we design a dynamic transmission controller to continuously calibrate neural codec configurations at runtime. It contains a \textit{codec configuration calibrator} that operates based on an offline profiled look-up table (LUT), a \textit{content-aware tile selector}, and a \textit{lightweight bandwidth estimator}.

\subsubsection{Adaptation Problem Formulation}
The adaptation objective is to maximize offloaded DNN accuracy on each frame satisfying the real-time latency constraint under certain bandwidths. To do so, a LUT is first created offline as $\bm{\{keys:[C_i],values:[(P_i,B_i)]\}_{i=1}^n}$
where $\bm{C_i}$ is the codec configurations, $\bm{P_i}$ and $\bm{B_i}$ are the corresponding profiled task accuracy and bandwidth consumption. $\bm{B_i}$ is calculated by $\bm{B_i=FS_i/T^t_i}$ where $\bm{FS_i}$ and $\bm{T^t_i}$ are the average tile size and a predetermined transmission time threshold. 
If the profiled bandwidth consumption of a configuration is higher than the estimated network bandwidth, the transmission time can exceed the threshold leading to system lagging and stuttering.
% 
At runtime, a content-aware tile-in-frame selection is performed first, giving a list of selected tiles $\bm{LT}$, and the numbers of selected tiles $\bm{t_s}$. Meanwhile, an estimated available bandwidth $\bm{EAB}$ is given by a lightweight estimator. Then the objective of adaptation can be evolved into finding the codec configuration $\bm{C_i}$ with the best task accuracy $\bm{P_i}$ that fits $\bm{B_i<EAB}$.


\subsubsection{Offline Profiling}
% \shengzhong{First introduce where the offline profiles are used. Explain what we need to profile for what configuration, and what dataset is used (in what portion and scale). How many times do you need to run in profiling? How the results are saved in your profiles? For example, in your LUT, what are the keys of the table, and what are the values of the table?}
To prepare the aforementioned LUT, we use a small profiling data set from the ABO RAW dataset (details in Appendix \ref{apdx:rawdataset}) to measure the average accuracy and tile size. 
The throughput of codec configurations is obtained by running on live cameras under certain bandwidth constraints without involving the dynamic transmission controller.
% Each FPS value recorded in the LUT will be the average result of 10 different camera positions.


\subsubsection{Bandwidth Estimation}
% \shengzhong{Since this is not our new contribution, use a very short paragraph to explain what you do.}
% To select codec configuration more precisely based on the result of tile-in-frame selection, 
We use a lightweight bandwidth estimator to obtain the estimation of the currently available bandwidth (EAB). 
The estimation $\bm{BW}$ is obtained by a simple time differential
$\bm{BW =\frac{S_{trans}}{t_{end}-t_{start}}}$
where $\bm{S_{trans}}$ is the transmitted bit-stream size of the last frame, $\bm{t_{start}}$ and $\bm{t_{end}}$ are the starting and ending timestamp of transmission of the last frame.

\input{algorithm/adaptation}

\subsubsection{Content-Aware Tile Selection}
To enhance content awareness in tile selection, we use detection results from the latest frame as references for tile selection in the next frame.
% Denote the area of the bounding boxes from the inference result of the last frame as $\bm{\{bbox_1,bbox_2,\cdots,bbox_m\}}$, assuming there are $\bm{m}$ detected objects. For a tile $\bm{T}$, if one of the bounding box areas $\bm{bbox_i}$ meets $\bm{T\cap bbox_i\neq \varnothing}$, then the tile $\bm{T}$ is selected for encoding and transmission. 
For each new tile, if it overlaps with any object bounding boxes in its previous frame, it will be selected for encoding and transmission. 
Such a conservative criteria ensures only tiles that are unlikely to contain objects are skipped.
However, if previous detection results are inaccurate, the following tile selections could be affected in a cascade.
To avoid this case, we use a periodic method to reset potential reference errors in fixed-length time windows.
In each window, the first frame is always encoded with all tiles in the highest configuration (called the \textit{key frame}), while the following frames are encoded with tile selection and codec configuration calibration. 
Since key frame transmissions only happen in low frequencies, their overhead is attenuated across all frames in the window and potential reference error accumulation is upper bounded, thus we guarantee the reliability of tile selection with high throughput and low latency even in high-motion scenarios.

\subsubsection{Adaptation Algorithm}
With the above definitions, the adaptation algorithm can be described as shown in Algorithm~\ref{alg:adaptation}.
For a given frame, if it is the first frame of a controlling window (a key frame), all the tiles will be encoded in the highest configuration and transmitted for DNN inference. The inference results will be stored as a reference. If it is not a key frame, the tile selection will be performed first. For each tile in the frame, if it is not already selected and has a cross-section with any bounding box from the last frame inference results, it will be selected for encoding and transmission. After the tile selection is finished, the number of selected tiles will multiplied by the bandwidth usage profile to obtain the estimated bandwidth request (EBR). The best configuration with an EBR less than the EAB will be used for encoding selected tiles and the DNN inference results will be used for tile selection of the next frame.
% The calibration of codec configuration is a collaborative work of offline profiler, content-aware tile selection, and online bandwidth estimator. The offline profiled LUT and tile selection results contribute together to the estimated frame bandwidth estimation. By comparing it with the estimated available bandwidth, the codec configuration with the highest task accuracy among the ones that fit below the predetermined transmission time threshold is chosen. Using a controlling window further improves the robustness under long-term services.


\begin{figure}[t!]
    \centering
    \includegraphics[width=0.85\linewidth]{figure/4/prototype-v2.pdf}
    \vspace{-0.3cm}
    \caption{3D-printed AR offloading testing platform.}
    \label{fig:prototype}
\end{figure}







==> comment/3_framework_old.tex <==
\section{The \model~Framework} 
\label{sec:framework}
Here we first give an overview of the \model framework, then introduce the design details of each component.

\begin{figure}
    \centering
    \includegraphics[width=1\linewidth]{figure/3/3-1-mod5.pdf}
    \caption{\model Framework Overview}
    \label{fig:overview}
\end{figure}

\subsection{Overview}
As shown in Figure~\ref{fig:overview}, our framework contains two main components:

\textbf{Configurable RAW Neural Codec:}
It will compress the full-size RAW image into several feature maps block by block that have smaller physical dimensions and use less bandwidth while being transmitted to the server for reconstruction. The codec has multiple operation configurations to serve different weights of balance between bandwidth and task accuracy.

\textbf{Dynamic Transmission Controller:}
Before encoding a frame and sending it to the server, the controller decides which blocks of the frame have the actual targets and need to be transmitted. Based on the result and runtime bandwidth estimation, the controller selects a configuration for the codec that balances task performance and bandwidth consumption and sends the corresponding feature maps of selected blocks to the server. 
In theory, the controller operates on a per-frame basis.

\subsection{Configurable RAW Neural Codec}
% \shengzhong{Need a diagram to visualize the tile/block-based compression idea. Do not address the ``adaptive'' here, but instead address that your codec supports dynamic configuration under different bandwidth constraints.}

\begin{figure}[t!]
    \centering
    \includegraphics[width=1\linewidth]{figure/3/tiles.pdf}
    \caption{The Tile-Wise Encoding of \model}
    \label{fig:tiles}
\end{figure}

As discussed in Section~\ref{sec2-1}, a single RAW frame without any encoding and compression has a transmission size of 6MB, around 200KB even with the entropy coding technique, which is not affordable in an unstable wireless network situation even with just 1/3 of the theoretical data amount of JPEG. This is because, unlike JPEG, RAW images do not have any existing method with scalable compression ability to reduce the bandwidth overhead. For that matter, we proposed a new adaptive neural codec of which the backbone model is based on DeepCOD\cite{yao2020deep}. 
The codec is operated in a block manner, encoding and decoding one small area of the full image at a time. Specifically, 3 blocks in a row and 4 blocks in a column, making 12 blocks of each frame. This will allow the dynamic transmission controller to select only the useful area of a frame, reducing both encoding overhead and bandwidth consumption. Also, spatial overlay among the blocks is introduced while splitting a frame to avoid the deflection on the edges of blocks caused by fixed padding. 
Inspired by EfficientNet\cite{tan2019efficientnet}, the adaptation of our codec is designed to be controlled by the width and depth of the encoder. The out depth of the encoder can be chosen between 8 and 4 channels, and the encoding convolution stride can be chosen between 2 and 4, making 4 different configurations total. For the decoder, only the first layer which is a residual deconvolution block is not shared. 
% More configurations can be added, but to our observation, 8 channel output with convolution stride set to 2, which is the largest and best configuration, is sufficient for YOLOv5. Any configuration with a larger encoded feature map size will only negligibly increase the task accuracy but result in a huge bandwidth overhead increase.

% \begin{figure}
%     \centering
%     \includegraphics[width=1\linewidth]{figure/3/3-1-mod2.pdf}
%     \caption{Overview of the \model~framework}
%     \label{fig:overview}
% \end{figure}

\begin{figure*}
    \centering
    \includegraphics[width=1\linewidth]{figure/3/3-3-mod.pdf}
    \caption{The configurable image neural codec in \model. \shengzhong{Compress the height}}
    \label{fig:modelstruct}
\end{figure*}

Unlike the input form of full-size raw we used in the motivation experiment, since the encoder is a one-layer convolution architecture, if the raw image were to be put straight into the encoder, the grid-like RGB information would be erased by the convolution kernel and making the reconstruction of color impossible. Instead of directly using the 1-channel RAW image as input, we disassemble an image by the CFA color channel and stack them on each other to create a 4-channel input (illustrated in Figure~\ref{fig:4into1}), so that the color information of each channel can be reserved after the decoding process and reassembled back to full resolution with the same amount of input data. After the blocks are decoded on the edge server, they still need to be reassembled back into the original 1-channel form with a grid-like color channel arrangement same as the original RAW frame. This is because though the amount of data and contained information of a frame are the same, the width and depth of the downstream DNN model will be influenced by the change of input shape, therefore impacting the sheer performance of the DNN model itself.

% distillation
The loss function of adaptive codec training is MSE, which only represents reconstruction quality. Presume there are $n$ train samples in total, and $y_i$ is the codec output of corresponding ground truth input $x_i$, then the MSE loss function can be described as follows:
\begin{equation}
MSE=\frac{1}{n}\sum_{i=1}^{n}(x_i-y_i)^2
\end{equation}
As discussed previously, the purpose of a machine-centric system is not a better reconstruction ability (hence a better QoE) but the best task performance. To that end, we introduced knowledge distillation\cite{distill} into the training procedure of the adaptive codec. 
% The purpose of regular knowledge distillation is to produce a smaller model supervised by the larger target one so that the smaller model will have a similar inference output and performance as the target model. 
In \model, the purpose of knowledge distillation is to fine-tune the adaptive codec so that the decoded image can trigger the downstream DNN model to produce better inference results.
After being trained respectively, the codec and the downstream vision model are assembled to create a full inference pipeline. Fine-tune of the codec will run within this pipeline. To be more specific, the parameter of the downstream DNN model will be frozen, and the optimizer used in this step will only update the parameters of the adaptive codec. Instead of using the original loss function, which represents only the quality of reconstruction, the loss function from the training procedure of the downstream vision model will be used here to guide the fine-tuning of the adaptive codec, since the design of \model~is machine-centric and the inference result is all that matters here. 
The multiply parameter, or the proportion of the knowledge distillation loss function for four different configurations of the adaptive codec is determined by the proportion of original MSE loss. As shown in Equation 1, after multiplying the parameter, all four configurations of adaptive codec should have the same loss value at the beginning of knowledge distillation to make all four configurations be updated at a similar speed rate. The proportion of loss function for each configuration can be described as follows:
\begin{equation}
P_i=\frac{\sum_{i=1}^{4}Loss_i}{Loss_i}
\end{equation}


\begin{figure}
    \centering
    \includegraphics[width=1\linewidth]{figure/3/3-2.pdf}
    \caption{Color-preserving input preprocessing.}
    \label{fig:4into1}
\end{figure}

\subsection{Dynamic Transmission Controller}
\label{3.3}
In typical AR scenes, not all the areas of a frame are related to the task. Thus, that unwanted area, or backgrounds, can be ignored during encoding and transmission to reduce bandwidth consumption while keeping the task performance unharmed. After the blocks are transmitted, the missing area can be simply filled with the same data used in the regular data processing pipeline for padding. Notice that after the blocks are decoded, they need to be assembled back into a one-dimension form which is the same as the original RAW image, and used in the downstream vision task.

\subsubsection{Offline profile}
\label{sec3.3.1}
To match the current bandwidth limitation while maintaining as high a performance of the vision task as possible, an offline profile needs to be created to find the Pareto limit. A part of a custom RAW dataset (details in ~\ref{rawdataset}) is utilized for this purpose. Measured results are shown in Figure~\ref{fig:pareto}. Our codec outperforms JPEG throughout the entire frame size range of the transmitted feature map on both mAP and F1 scores. Similar to JPEG, the highest configuration does perform the best, but the improvement may not match the overhead of bandwidth consumption, so it may only be used when bandwidth is sufficient to further improve QoE. The measurement results will be used for the algorithm design in the transmission controller later.

\begin{figure}
    \centering
    \includegraphics[width=1\linewidth]{figure/3/pareto.pdf}
    \caption{Measured Pareto boundary of JPEG and Our framework on a custom RAW dataset}
    \label{fig:pareto}
\end{figure}

\subsubsection{Object-location-based transmission controller}
\ 
The controller provides two main functions: block \& frame selection and codec configuration selection.

\textbf{Block \& frame selection} 
The most simple way to reduce transmission overhead is to only use the wanted area of a frame. As introduced previously, the adaptive RAW codec is operated block by block, so that the first thing needs to be decided is which blocks of a frame need to be transmitted, or even which frames. The selection has to run sequentially with encoding and transmission, meaning that the computation must be lightweight enough to be run on edge devices in real-time tasks. The simplest way is to directly calculate the mean square error (MSE) of each block, if the MSE is larger than a pre-determined threshold, the corresponding block will not be encoded and transmitted. However, using only the MSE threshold may cause using unwanted blocks due to changes in background, or missing wanted blocks with a small part of the target but not triggering the threshold. An alternative method is optical flow, which tracks the moving vector of pixels and creates a vector matrix to show which part of a frame is moving, as well as the direction and moving speed. But, same as the limitation of debayering high-resolution frames, with such a huge amount of pixels, running optical flow is too slow to run on mobile devices for real-time tasks. On our test platform, Jetson Nano, it takes over 25 ms to perform optical flow calculation for just one frame, which is far from acceptable in real-time AR/VR applications.
Since the first frame in a stream is always being fully transmitted, the result from it can be used as a reference for transmission control of upcoming frames. A controlling window length will be determined before a stream starts, the first frame of a controlling window will be encoded and transmitted to the server without any blocks dropped, and act as the key frame of this controlling window. All the other frames within this controlling window will use the result from the key frame. Furthermore, if there are not any targets in the key frame, all the following frames within keyframe rolling window will not be encoded or transmitted and only be rendered for display on the client device. Unlike FFMPEG\cite{tomar2006converting}, in which parameters like bit rate and key frame interval of a given segment are predetermined by the user, our framework can be operated frame by frame and the controlling window can be changed dynamically as desired.

\textbf{Available bandwidth estimation}
To select codec configuration more precisely based on the result of block \% frame selection, a bandwidth estimation mechanism needs to be utilized. The transmitted bit-stream size of the last key frame is a known value $S_{trans}$, ankeyframeulating the differential of time stamp, the transmission interval of the last key frame can also be obtained by $T_{trankeyframe}-t_{start}$ so that the available Bandwidth estimation can be represented as:
\begin{equation*}
Bandwidth=\frac{S_{trans}}{t_{end}-t_{start}}
\end{equation*}
Instead of using prediction methods like a regressive algorithm, a simple maneuver can still provide accurate bandwidth estimation without introducing extra calculation overhead.

\textbf{Codec configuration selection} 
After obtaining the estimation of available bandwidth, the configuration of the codec can be selected. Unlike JPEG, which is a spatial compress method and the outcome size of which can differ vastly between different complexities of content in the frame, the compress of \model~is based on entropy coding (detail in section\ref{sec4.2}) meaning the encoded and compressed size of frames using a given codec configuration will sit in a relatively stable interval. Based on the measured results in section\ref{sec3.3.1}, a bandwidth consumption estimation look-up-table (LUT) of each codec configuration can be created. The transmission controller will always choose the best configuration that satisfies the bandwidth estimation after considering the results from block \& frame selection.








==> comment/4_implementation.tex <==
\section{Implementation}\label{sec:implementation}
\subsection{Hardware Prototype}
As shown in Figure~\ref{fig:prototype}, we build a hardware prototype system with a 3D-printed AR goggle modified from Google Cardboard~\cite{cardboard}.
We use two IMX178 rolling-shutter sensors from SonySemicon~\cite{hikcamera} as cameras, with a solution of $3072\times2048$ and a maximum frame rate of 60 FPS. 

We use NVIDIA Jetson Nano as the edge device for onboard processing. 
The edge server is configured with an AMD Ryzen R9-7950X CPU with a Nvidia RTX4090 GPU and 64GB RAM, comparable to home desktop PCs. 
The client device and the edge server are connected 
through a 200 Mbps wireless network.

\subsection{Software Implementation}
\label{sec4.2}
We implemented \model framework with 4500 LoC Python code, using PyTorch 2.0~\cite{paszke2019pytorch} as the DNN platform. The network connection and data transmission is achieved through the TCP Socket protocol. The downstream object detection model is YOLOv5-7.0.
Encoders on the edge device are converted to FP16 TensorRT engines~\cite{tensorrt}. Lempel-Ziv coding and Huffman coding are employed for data compressing before transmission to further reduce bandwidth consumption.

\subsection{System Optimizations}
\subsubsection{Pipelining.} 
The pipeline of \model implementation is illustrated in Figure~\ref{fig:pipeline}. Multi-threading the demosaic process with the others means the execution time of all the processes except encoding will be extended since the total CPU resource pool is very limited. However, according to our observation, the multi-threaded pipeline still provides 15\% more FPS with 17\% less end-to-end latency compared to a sequential one.

\subsubsection{Quantization.} 
We reduce bandwidth consumption by quantizing the encoded feature map into unsigned INT8 using simple \textit{add} and \textit{mul} operations. The parameter of quantize is obtained from the upper and lower bound of encoded feature maps of the training set. The quantization brings only about 0.05\% degradation of task performance with a neglectable processing time overhead and a reduction in bandwidth consumption of about 75\%. 
% We have also investigated the possibility of using even more aggressive quantization precision, like unsigned INT4 (0-16), which will further reduce the bandwidth consumption to just 8\% of using FP32. However, since the workflow used in \model~does not support uint4 natively, it has to be done by bit shifting of two nearby data and packaging them into uint8. Despite that such a maneuver will not significantly increase end-to-end latency since the processing is fast enough, it does harm the task accuracy to an extreme point, degrading from over 0.9 to under 0.2. So in our implementation, we stick with the uint8 solution.

\begin{figure}[t!]
    \centering
    \includegraphics[width=0.95\linewidth]{figure/4/4-1-mod4.pdf}
    \vspace{-0.2cm}
    \caption{\model framework operational workflow.}
    \label{fig:pipeline}
\end{figure}

==> comment/5_experiment.tex <==
\section{Experiments} \label{sec:experiment}
% In this section, we present extensive experiments conducted on a newly collected and labeled RAW dataset to evaluate the performance of the proposed framework. 
% In this section, we commence describing the experimental setups and the datasets employed in our experiments. Then, we provide a comprehensive comparison of overall performance against various baseline methods, followed by robustness evaluation, ablation study, and robustness evaluations.

\subsection{Experimental Setups}
\label{sec:setup}
\subsubsection{Dataset.}
% \shengzhong{We still need short introduction of the used dataset.}
% Common image datasets do not contain RAW format before demosaicing. We need to use dedicated camera sensors to collect data to preserve RAW images and demosaiced RGB images. More details about the dataset are introduced in Section~\ref{rawdataset}
Since existing public datasets do not contain RAW image frames, we manually collect segments of 10-40 seconds consecutive RAW frames at 30 FPS using the prototype AR device, including different possible real-world AR scenarios. The detailed statistics are summarized in Appendix~\ref{apdx:rawdataset}.
% Since existing public datasets do not contain RAW image frames, we manually collect segments of RAW frames at 30 FPS using the prototype AR device, including different possible real-world AR scenarios.

\subsubsection{Evaluation metrics}
To verify the performance of the proposed framework, we consider the following metrics perspectives.
\begin{itemize}
    \item \textbf{Task Accuracy:} 
% In a machine-centric scenario, the accuracy of the downstream DNN vision task can be used to reflect the performance of the encoder-decoder set. 
For the object detection task, mean average detection precision (mAP)~\cite{everingham2015pascal, lin2014microsoft}, F1 score, precision, and recall are used to represent the overall task accuracy.
    \item \textbf{Frame Processing Latency:} 
% AR/VR scenario is known to be sensitive to latency as the frame rate is a major metric of the human viewing experience. 
It is defined as the duration from the frame being captured to the remote detection results being rendered and displayed by the client device.
    \item \textbf{Throughput:} 
% Since in the practical pipeline, there will be some steps that can be stacked on each other with multi-threading, the final presented frame per second (FPS) will not simply be the reciprocal of the frame time. Therefore, the final FPS is used to verify the optimization of throughput.
The frame processing throughput is critical to the smoothness of the user experience. 
It is defined as the number of frames that are processed per second.
    \item \textbf{Bandwidth Consumption:}  
% Reduced bandwidth demand will provide a better frame latency which means higher throughput under an unideal network. 
% Also, the conflict between reducing bandwidth consumption and maintaining task accuracy always exists. 
% The bandwidth consumption will used along with task accuracy to evaluate the Pareto limit of different frameworks.
It measures the average size of transmitted frames, as network bandwidth has become one of the resource bottlenecks in edge offloading.
\end{itemize}

\subsection{Compared Baselines}
We compare with the following baselines in our experiments:
\begin{itemize}
    \item \textbf{JPEG~\cite{wallace1992jpeg}:} One of the most widely used methods of lossy compression for RGB images, with a scaled compression ratio reflecting the tradeoff between image quality and file size. We set the JPEG configuration with an adaptive encoding quality module according to the available bandwidth. 
    \item \textbf{DeepCOD~\cite{yao2020deep}:} A neural offloading framework using different layers of deep compression model to achieve efficient transmission while balancing reconstruction quality and downstream task accuracy. 
    \item \textbf{PNC~\cite{wang2023progressive}:} An adaptive neural offloading framework achieving selectable compression level via stochastic tail-drop according to the importance of the feature map layers. 
    \item \textbf{Reducto~\cite{li2020reducto}:} An adaptive frame selection offloading framework with a per-frame differential extractor on the client and offline profiles for scenarios on the server to control which frames to transmit within a stream. 
\end{itemize}

\subsection{Offline Accuracy Profile}

\begin{figure*}[t!]
\centering
\begin{minipage}{.47\linewidth}
  \centering
    \includegraphics[width=1\linewidth]{figure/5/profile_acc_v2.pdf}
    \vspace{-0.6cm}
    \caption{Accuracy and frame size profiles.}
    \label{fig:profile acc}
\end{minipage}
\begin{minipage}{0.02\linewidth}

\end{minipage}
\begin{minipage}{.47\linewidth}
  \centering
    \includegraphics[width=1\linewidth]{figure/5/profile_lat_v2.pdf}
    \vspace{-0.6cm}
    \caption{Throughput \& latency under 20 Mbps bandwidth.}
    \label{fig:profile lat}
\end{minipage}
\end{figure*}

\begin{figure*}[t!]
    \centering
    \includegraphics[width=0.94\linewidth]{figure/5/overall_acc_v2.pdf}
    \vspace{-0.3cm}
    \caption{Adaptation accuracy under bandwidth dynamics.}
    \label{fig:overall acc}
\end{figure*}

\begin{figure}[t!]
    \centering
    \vspace{0.2cm}
    \includegraphics[width=0.9\linewidth]{figure/5/overall_speed_v2.pdf}
    \vspace{-0.3cm}
    \caption{Adaptation efficiency under bandwidth dynamics.}
    \label{fig:overall speed}
\end{figure}

An optimal neural codec should reduce the frame into smaller sizes while sustaining higher downstream task accuracy.
We therefore measure the accuracy and bandwidth tradeoffs between different configurations in offline profiling, which represents the Pareto boundaries of the compared frameworks.
Specifically, for each configuration, we measure the task accuracy metrics after decoding and the average compressed frame sizes across the test segments as shown in Figure~\ref{fig:profile acc}.
Each line represents a framework and each point represents a concrete configuration.
\model reaches the highest Pareto limit among all frameworks across all configurations. 
Compared with the JPEG pipeline, \model has an over 15-20\% better task accuracy while only using 30-50\% less bandwidth, demonstrating the importance of task-aware end-to-end code training in DNN offloading.
Besides, although based on the same model architecture, \model outperforms the frame-level encoding of DeepCOD significantly benefiting from its tile-wise encoding and object-free tile filtering during encoding.
Finally, the sole frame selection in Reducto presents poor bandwidth efficiency in downstream tasks.
% The largest and most accurate configuration of DeepCOD has a smaller bandwidth usage only because it has a nearly twice smaller data dimension ($16\times102\times152$ compared to $12\times8\times35\times39$). 
% However, not only it does not achieve a twice smaller bandwidth usage, which the second best configuration of \model~(also has a twice smaller data dimension) does, but also the task accuracy does not match with the second best configuration of \model. The other baselines, whether learn-based or not, simply can not beat \model on both task accuracy and bandwidth consumption across all configurations. So it can be concluded that \model has achieved Pareto optimality.
% \vspace{-0.8cm}
\subsection{Offline Throughput and Latency Profile}
The end-to-end frame processing latency and the throughput under limited bandwidth are directly related to the responsiveness and smoothness of user experience. 
Therefore, we upper bound the wireless network to 20 Mbps and measure the above two metrics for different configurations within each framework, using all collected test segments.
As illustrated in Figure~\ref{fig:profile lat}, under the same frame sizes, \model achieves the highest throughput and the lowest end-to-end latency, being the only framework surpassing the 25 FPS threshold of real-time inference, demonstrating that the advantages of \model also come from its higher client-side computation efficiency and system pipelining.
Compared to the JPEG pipeline, \model increases the throughput by 50\% while reducing
the end-to-end latency by 35\%, highlighting the savings by parallel demosaicing and DNN offloading. 
% Decoupling demosaic process and offloading processes is time-saving and latency-friendly by nature, and the dynamic offloading controller further reduces the redundancy of transmitted data and optimizes the throughput and end-to-end latency. 
PNC struggles with 15\% lower throughput and 10\% higher latency than JPEG, despite its channel-dropping effort, because its encoder still has a large scale that leads to high computation overhead. 
Other baselines have only improved 3\% to 15\% of throughput and 5\% to 10\% of end-to-end latency compared to JPEG without refactoring the underlying codec.

\subsection{Adaptation Performance}

We further perform end-to-end comparisons when individual configurations are integrated into an adaptive framework under network dynamics. 
To conduct the adaptation experiments in a reproducible way, we use both randomly generated and real-world recorded network bandwidth traces~\cite{kan2022improving} (as summarized in Appendix~\ref{apdx:bandtrace}) and replay the network traces to each video segment and each framework, respectively. The network bandwidth is dynamically bounded using Linux Traffic Control (tc)~\cite{linuxtc}.
The results are shown in Figure~\ref{fig:overall acc} and Figure~\ref{fig:overall speed}. \model consistently outperforms the baselines in both downstream task accuracy and frame processing throughput. 
% except in segment 4, ABO has gaps of 0.07\% on F1 score and 0.03\% on mAP from DeepCOD. This is because in order to save the execution time on the server, we did not utilize any self-attention module in the decoder which DeepCOD did, hence the neglectable performance drop in test segment 4. 
Neural encoding frameworks generally achieve better task performance (\model, DeepCOD, and PNC), where \model demonstrates the best efficiency and accuracy tradeoff. 
DeepCOD and Reducto deliver increased throughput than JPG but still can not meet the smooth browsing requirement (\ie > 25 FPS). 
PNC suffers from long encoding time although the transmitted frame sizes are compressed through its channel-dropping strategy.
In AR applications, since objects are mostly in high motion to the user, the frame selection in Reducto leads to poor downstream accuracy.
Finally, \model~also achieves the lowest end-to-end latency, thanks to its demosaic-free offloading pipeline. 
In summary, the results prove that \model provides the highest quality with guaranteed responsiveness and smoothness to the users.

\subsection{Environmental Robustness}
We evaluate two challenging scenarios in AR applications that require higher robustness (details expanded in Appendix~\ref{apdx:capability}). 

\subsubsection{Low-Light Scenario}
We manually change the luminosity scale of the collected video frames from 1 to 1/2 and 1/4, and compare the accuracy degradation between \model and JPEG codec on their highest configurations.
As shown in Figure~\ref{fig:luminosity}, when operating in low-light conditions, \model achieves lower accuracy degradation below 0.1 while JPEG has an unbearable 0.35 at 1/4 luminosity.

\subsubsection{High-Motion Scenario}
% Active user interactions make motion blur common in AR. Therefore, 
We separately analyze the downstream accuracy of two video segments (\ie Seg3 and Seg5 ) that were collected with higher camera motions.
As shown in Figure~\ref{fig:motionblur}, neural codecs solutions tend to have better robustness than frameworks with standard JPEG encoding. 
Besides, \model outperforms the baselines with a larger margin than overall evaluations in Figure~\ref{fig:overall acc}, being the only framework to sustain over 0.85 mAP in both videos.

\begin{figure}[t!]
    \centering
    \includegraphics[width=1\linewidth]{figure/5/luminosity_v2.pdf}
    \vspace{-0.7cm}
    \caption{Accuracy degradation under low luminosity.}
    \label{fig:luminosity}
\end{figure}

\subsection{Ablation Study}
To inspect the optimization brought by each module, we designed two ablation experiments. One removes the distillation process in the offline codec training, while the other one removes the tile selection module in dynamic transmission control.
The results are shown in Table~\ref{tab:ablation}. 
Knowledge distillation does not affect frame size, throughput, or end-to-end latency, but brings a huge improvement in task accuracy (over 5\% mAP), making it an essential component in \model. 
Besides, tile selection saves 23\% in average frame sizes with on average 29\% tiles dropped, hence the improvement in throughput and latency, without degrading the downstream accuracy.

\begin{figure}[t!]
    \vspace{0.2cm}
    \centering
    \includegraphics[width=1\linewidth]{figure/5/motionblur.pdf}
    \vspace{-0.7cm}
    \caption{Adaptation performance in high-motion videos.}
    \label{fig:motionblur}
\end{figure}

\subsection{Overhead Quantification}
% \shengzhong{Report the overhead in cumulative distribution curve (CDF). Include both the memory and power consumption overhead.}
% To quantify the memory usage and energy overhead of \model to evaluate its applicability in mobile AR devices.
To evaluate the applicability of \model in mobile AR devices,
we monitor the power and memory usage throughout the testing periods. 
The Power consumption is measured with a Monsoon HV power moniter~\cite{hvpm} at 0.2 ms intervals. 
% The memory usage is measured from 20 runs of the former experiments.
The cumulative overhead distribution curves of JPEG and \model are visualized in Figure~\ref{fig:overhead}.
% For the JPEG pipeline, the average power consumption of the client device is 9.5W. For \model, it is 10W, increased by less than 10\%, which is within a reasonable range considering our implementation has a higher performance utilization ratio. 
% In power consumption, the average power of \model is 10 W, which increases by < 10\% than 9.5 W of JPEG, demonstrating its high power efficiency.
% In memory usage, after utilization, \model consumes 1080 MB of memory while JPEG consumes 340 MB. 
In energy overhead, the average power of \model is 10 W, which increases by < 10\% than 9.5 W of JPEG, demonstrating its high power efficiency.
In memory usage, after initialization, \model consumes 1080 MB of memory while JPEG consumes 340 MB. 
This is reasonable since we host multiple neural encoders on the edge device, but its absolute memory consumption is acceptable to current AR device capacities.




==> comment/dataset.tex <==
\section{Dataset Details}
\label{apdx:rawdataset}

In our experiments, the downstream vision task deployed on the server is YOLO-based object detection. Existing common datasets \cite{lin2014microsoft,deng2009imagenet} are all collected and labeled with RGB standards like JPEG, and simulating RAW images from such data is nearly impossible. On the other hand, existing RAW datasets \cite{abdorgchen2018learning, dong2022abandoning, kodak} either simply do not have the sufficient amount of images to create a persuading test environment, or are not designed for vision tasks but only compressive encoding. Thus, for experiments, we construct a new RAW dataset, the \model RAW dataset, with 17 types of common objects in campus offices, containing over 10,000 images with high-quality labeled bounding boxes. All the images are captured with a resolution of 3072*2048 under 8-bit non-packing Bayer mode with the digital gain set to zero to reduce any possible noises and secure image quality.
This dataset is designed not only to serve the object detection task but also to improve the robustness under common challenges in AR/VR scenes like dim light or motion blur. To make the proxy of AR/VR scenario more viable and improve the robustness, random movements of the camera and objects are introduced during the data collection process to improve the tolerance of motion blur in real-life AR/VR scenarios. Roughly 5\% of the total dataset is collected under insufficient luminosity conditions to robustness under indoor environments. We also introduced several frames of pure black and white for gamma calibration.

However, the dataset is collected one frame at a time to maintain the variety of samples, meaning it cannot be used as frame streams since the frames are not consecutive. To evaluate the framework, we also collected 5 segments of consecutive frames at a fixed frame rate of 30 FPS using the prototype AR device. The segments include different possible real-world AR/VR scenarios within time lengths varying from 10 to 40 seconds, simulating both short-burst and long-term services.

% \textbf{Data Processing} Since the downstream visual task does not need a full-resolution frame, frames need to be down-sampled before being transmitted. For RAW frames, this can be simply done by grid selection of the original data which still can keep the nature of directly sampling the real world, merely with a smaller sample rate. However, on the JPEG side, different orders of down-sampling and demosaicing operations will result in slightly different results. In a normal JPEG pipeline, a CFA image is demosaic first, then a bi-linear down-sample will be performed to resize the demosaiced RGB image into a desired size. However, if the down-sample on RAW is performed first since the spatial sample rate is not the same as the original. This may cause a moire pattern in the images (as shown in Figure~\ref{fig:moire pattern}) which will deflect the image quality and affect task performance. In our experiments, all the training and evaluation images will be processed as the same in the regular JPEG pipeline.

% \begin{figure}
%     \centering
%     \includegraphics[width=1\linewidth]{figure/5/moire.pdf}
%     \caption{Using Alternative pipeline will affect the outcome while using JPEG\textcolor{red}{need to be more obvious, illustrate with pipeline}}
%     \label{fig:moire pattern}
% \end{figure}

==> table/rebuttal_1.tex <==
\begin{table}[t!]
    \centering
    \caption{\model ablation study results.}
    \vspace{-0.3cm}
    \label{tab:ablation}
    % \tabcolsep=0.2cm
    \resizebox{\textwidth}{!}{%
    \begin{tabular}{c|ccccc}%{@{}c|ccc@{}}
    \toprule
      & Demosaic & Preprocessing & Encoding & Transmission & Server Processing & Result Renders \\ \midrule
    ABO & Hiden in parallel processing & 7.0 & 13.1 & Hiden in parallel processing & 4.1 (partially hiden in parallel processing) & 13.1 \\ 
    JPEG & 23.4 & 9.0 & 8.8 & 10.9 & 4.2 & 12.4 \\
    DeepCOD & 22.6 & 8.7 & 3.1 & 6.7 & 4.7 & 9.8 \\
    PNC & 23.8 & 10.0 & 9.6 & 7.2 & 5.1 & 11.3 \\
    Reducto & 23.6 & 9.2 & 8.9 & 8.7 & 4.2 & 12.7 \\ 
    \bottomrule
    \end{tabular}%
    }
\end{table}

==> text/7_discussion.tex <==
\section{Discussion} 
\label{sec:discussion}

% In this section, we briefly discuss the limitations in the current framework, and potential future directions that could be explored to extend the work.

There is still some room for improvement in our framework. For instance, the possibility of using different encoding configurations within one frame using a lightweight content-aware module remains, meaning that the bandwidth consumption can be further reduced.

==> text/motivation.tex <==
\section{Motivation:} \label{sec: motivation} 


